Ranking-Based Autoencoder for Extreme Multi-label Classification

Extreme Multi-label classification (XML) is an important yet challenging machine learning task, that assigns to each instance its most relevant candidate labels from an extremely large label collection, where the numbers of labels, features and instances could be thousands or millions. XML is more and more on demand in the Internet industries, accompanied with the increasing business scale / scope and data accumulation. The extremely large label collections yield challenges such as computational complexity, inter-label dependency and noisy labeling. Many methods have been proposed to tackle these challenges, based on different mathematical formulations. In this paper, we propose a deep learning XML method, with a word-vector-based self-attention, followed by a ranking-based AutoEncoder architecture. The proposed method has three major advantages: 1) the autoencoder simultaneously considers the inter-label dependencies and the feature-label dependencies, by projecting labels and features onto a common embedding space; 2) the ranking loss not only improves the training efficiency and accuracy but also can be extended to handle noisy labeled data; 3) the efficient attention mechanism improves feature representation by highlighting feature importance. Experimental results on benchmark datasets show the proposed method is competitive to state-of-the-art methods.

==> ndcg.tex <==
\begin{table*}[h]
\resizebox{2.0\columnwidth}{!}{%
\begin{tabular}{ccccccccc}
\hline
\textbf{Dataset}                    & \textbf{Metrics} & \textbf{SLEEC} & \textbf{FastXML} & \textbf{PD-Sparse} & \textbf{FastText} & \textbf{Bow-CNN} & \textbf{XML-CNN} & \textbf{RankAE} \\ \hline
\multirow{3}{*}{\textbf{Delicious}} & n@1              & 67.59          & \textbf{69.61}   & 51.82              & -                 & -                & -                & 69.26           \\
                                    & n@3              & 62.87          & \textbf{65.47}   & 46.00              & -                 & -                & -                & 64.16           \\
                                    & n@5              & 59.28          & \textbf{61.90}   & 42.02              & -                 & -                & -                & 60.39           \\
\hline
\multirow{3}{*}{\textbf{Mediamill}} & n@1              & \textbf{87.82} & 84.22            & 81.86              & -                 & -                & -                & 86.53           \\
                                    & n@3              & \textbf{81.50} & 75.41            & 70.21              & -                 & -                & -                & 78.36           \\
                                    & n@5              & \textbf{79.22} & 72.37            & 63.71              & -                 & -                & -                & 75.28           \\
\hline
\multirow{3}{*}{\textbf{RCV}}       & n@1              & 90.25          & \textbf{91.23}   & 90.08              & -                 & -                & -                & 90.9            \\
                                    & n@3              & 88.86          & \textbf{89.63}   & 88.50              & -                 & -                & -                & 89.29           \\
                                    & n@5              & 89.49          & \textbf{90.33}   & 88.79              & -                 & -                & -                & 89.75           \\
\hline
\multirow{3}{*}{\textbf{IMDb}}      & n@1              & 51.37          & 66.45            & 66.84              & 69.55             & 66.59            & 75.55            & \textbf{75.91}  \\
                                    & n@3              & 49.75          & 67.14            & 64.84              & 68.47             & 67.26            & \textbf{74.02}   & 73.5            \\
                                    & n@5              & 54.43          & 71.72            & 69.69              & 72.99             & 72.07            & \textbf{78.48}   & 77.37           \\
\hline
\multirow{3}{*}{\textbf{EURLex}}    & n@1              & 79.26          & 71.36            & 76.43              & 71.51             & 64.99            & 76.38            & \textbf{79.52}  \\
                                    & n@3              & 68.13          & 62.87            & 64.31              & 63.32             & 55.03            & 66.28            & \textbf{68.76}  \\
                                    & n@5              & 61.60          & 58.06            & 58.78              & 58.56             & 49.92            & 60.32            & \textbf{62.33}  \\
\hline
\multirow{3}{*}{\textbf{Wiki10}}    & n@1              & \textbf{85.88} & 83.03            & 81.03              & 68.86             & 81.16            & 84.11            & 83.6            \\
                                    & n@3              & \textbf{76.02} & 75.35            & 62.62              & 56.72             & 56.14            & 73.52            & 74.78           \\
                                    & n@5              & \textbf{68.13} & 63.36            & 52.03              & 51.19             & 45.29            & 65.50            & 67.18           \\
\hline
\hline
\textbf{Rank Score}                 & \textbf{avg}     & 2.83           & 3.22             & 4.33               & 4.67              & 5.78             & 2.56             & \textbf{1.89}  
\\ \hline
\end{tabular}
}
\caption{$n@k$: nDCG at Top K. The '-' indicates unavailable and \textbf{bold} is the best result in the line.}
\label{tab:ndcg}
\end{table*}

==> noise.tex <==

% \subsection{Noise Tolerace}
% As mentioned in our method part, the proposed loss ranking is robust to label noise, by changing the margin range between $0$ to $1$. The larger the margin is, the less tolerated our model will be, vice versa. In order to demonstrate our ranking loss is more robust to label noises during training comparing with Binary Cross Entropy loss, we created two different types of noises:

% \textbf{Missing Label Noise}: With a label dropping rate, saying from $10\%$ to $40\%$, we will randomly drop the current labels in training set based on the rate. Then we created four new missing noised training data, with $10\%$, $20\%$, $30\%$ and $40\%$ label dropping rates. However, we leave the test as before. Then we tested both XML-CNN, which uses BCE loss, and our proposed model with ranking loss. As shown in Figure \ref{fig:missing}, in each sub-figure, the x-axis represents the label dropping rate, and y-axis is either $P@k$ on the top row or $nDCG@k$ at the bottom row. And each column stands for the top $k$s in the evaluation metrics, with increasing order from left to right. 

% In Figure \ref{fig:missing}, orange line stands for our method, while blue line is XML CNN. First, the XML-CNN and our method are very competitive to each other when dropping rate is lower than $20\%$. However, with keeping increasing dropping rate, XML-CNN shows dramatic drops in both $P@k$ and $nDCG@k$ for all $k$s. It is worth noting that, our method still produces well performed results even with $40\%$  dropping rate. In addition, the performance drop is surprisingly less than $10\%$ from the highest point for our method, while XML-CNN drops almost $50\%$ at $P@3$ and $nDCG@3$. 


% \text{Wrong Label Noise}: With very similar setups for creating missing labels dataset, we created the wrong label noise by 1) dropping some of tagged labels like before but at the same time, 2) injecting extra labels with some rate, from $10\%$ to $40\%$. Therefore, for these four new noised training data, we not only lose some positive labels but also obtain some inaccurate extra labels with same drop and injection rate. We tested our model and XML-CNN on this wrong label dataset. 

==> precision.tex <==

\begin{table*}[t]
\resizebox{2.0\columnwidth}{!}{%
\begin{tabular}{ccccccccc}
\hline
\textbf{Dataset}                    & \textbf{Metrics} & \textbf{SLEEC} & \textbf{FastXML} & \textbf{PD-Sparse} & \textbf{FastText} & \textbf{Bow-CNN} & \textbf{XML-CNN} & \textbf{RankAE} \\
\hline
\multirow{3}{*}{\textbf{Delicious}} & P@1              & 67.59          & \textbf{69.61}   & 51.82              & -                 & -                & -                & 69.26           \\
                                    & P@3              & 61.38          & \textbf{64.12}   & 44.18              & -                 & -                & -                & 62.72           \\
                                    & P@5              & 56.56          & \textbf{59.27}   & 38.95              & -                 & -                & -                & 57.63           \\
\hline
\multirow{3}{*}{\textbf{Mediamill}} & P@1              & \textbf{87.82} & 84.22            & 81.86              & -                 & -                & -                & 86.53           \\
                                    & P@3              & \textbf{73.45} & 67.33            & 62.52              & -                 & -                & -                & 70.17           \\
                                    & P@5              & \textbf{59.17} & 53.04            & 45.11              & -                 & -                & -                & 55.44           \\
\hline
\multirow{3}{*}{\textbf{RCV}}       & P@1              & 90.25          & \textbf{91.23}   & 90.08              & -                 & -                & -                & 90.9            \\
                                    & P@3              & 72.42          & \textbf{73.51}   & 72.03              & -                 & -                & -                & 72.82           \\
                                    & P@5              & 51.88          & \textbf{53.31}   & 51.09              & -                 & -                & -                & 52.05           \\
\hline
\multirow{3}{*}{\textbf{IMDb}}      & P@1              & 51.37          & 66.45            & 66.84              & 69.55             & 66.59            & 75.55            & \textbf{75.91}  \\
                                    & P@3              & 34.46          & 48.32            & 46.29              & 48.76             & 48.42            & 52.59            & \textbf{52.66}  \\
                                    & P@5              & 27.34          & 36.28            & 35.04              & 36.53             & 36.56            & \textbf{38.90}   & 38.48           \\
\hline
\multirow{3}{*}{\textbf{EURLex}}    & P@1              & 79.26          & 71.36            & 76.43              & 71.51             & 64.99            & 76.38            & \textbf{79.52}  \\
                                    & P@3              & 64.30          & 59.90            & 60.37              & 60.37             & 51.68            & 62.81            & \textbf{65.14}  \\
                                    & P@5              & 52.33          & 50.39            & 49.72              & 50.41             & 42.32            & 51.41            & \textbf{53.18}  \\
\hline
\multirow{3}{*}{\textbf{Wiki10}}    & P@1              & \textbf{85.88} & 83.03            & 81.03              & 68.86             & 81.16            & 84.11            & 83.6            \\
                                    & P@3              & \textbf{72.98} & 67.47            & 57.36              & 54.65             & 50.67            & 70.24            & 72.07           \\
                                    & P@5              & \textbf{62.70} & 57.76            & 44.10              & 47.61             & 36.03            & 59.87            & 62.07           \\
\hline
\hline
\textbf{Rank Score}                 & avg              & 2.83           & 3.33             & 4.56               & 4.56              & 5.78             & 2.56             & \textbf{1.78}  
\\ \hline
\end{tabular}
}
\caption{$P@k$: Precision at Top K. The '-' indicates unavailable and \textbf{bold} is the best result in the line.}
\label{tab:prec}
\end{table*}
